SEFRQO: A Self-Evolving Fine-Tuned RAG-Based Query Optimizer

Query optimization is a crucial problem in database systems that has been studied for decades. Learned query optimizers (LQOs) can improve performance over time by incorporating feedback; however, they suffer from cold-start issues and often require retraining when workloads shift or schemas change. Recent LLM-based query optimizers leverage pre-trained and fine-tuned LLMs to mitigate these challenges. Nevertheless, they neglect LLMs' in-context learning and execution records as feedback for continuous evolution. In this paper, we present SEFRQO, a Self-Evolving Fine-tuned RAG-based Query Optimizer. SEFRQO mitigates the cold-start problem of LQOs by continuously learning from execution feedback via a Retrieval-Augmented Generation (RAG) framework. We employ both supervised fine-tuning and reinforcement fine-tuning to prepare the LLM to produce syntactically correct and performance-efficient query hints. Moreover, SEFRQO leverages the LLM's in-context learning capabilities by dynamically constructing prompts with references to similar queries and the historical execution record of the same query. This self-evolving paradigm iteratively optimizes the prompt to minimize query execution latency. Evaluations show that SEFRQO outperforms state-of-the-art LQOs, achieving up to 65.05% and 93.57% reductions in query latency on the CEB and Stack workloads, respectively, compared to PostgreSQL.

==> discussion.tex <==
\section{Discussion and Future Work}
% In this section, we summarize {\oursystem}'s benefits and limitations, and discuss some possible future investigations.
In this section, we discuss {\oursystem}'s current limitations and the future potential investigation directions.

\noindent\textbf{Enhancing LLM Output Stability.}  
Although our system performs well overall, the LLM occasionally generates outputs that deviate from the required hint format. Consequently, additional normalization steps are necessary to ensure that the resulting query plans comply with strict syntactic and structural requirements, thereby maintaining consistency and reliability in deployment. As a next step, we plan to investigate output‑formatting tools~\cite{liu2024weformat1,liu2025beyondformat2,shorten2024structuredragformat3} to enforce structural consistency in LLM-generated outputs.

% \noindent\textbf{Knowledge Distillation:} 
% Distill larger LLMs's 
% Research into distilling transferable knowledge from large models into smaller ones may help reduce inference times while preserving performance, making the approach more suitable for production environments~\cite{liu2024ddkdistill1,yang2024llmdistill2,wang2024usingdistill3}. A large LLM with powerful GPU support shouldn't be assumed to be always satisfiable in production, especially mobile and edge situations.




% \noindent\textbf{Enhanced Execution Speed and Transferability:} {\oursystem} performs better than conventional baselines without the need to design query embeddings~\cite{marcus2021bao,yang2022balsa}. By leveraging fine-tuning and dynamic retrieval capabilities, the model successfully transfers optimization strategies across diverse workloads, even when database schemas differ, thereby enhancing adaptability and robustness.


% \noindent\textbf{Pipeline Latency Concerns:} 
% While overall speed is improved, the additional retrieval and inference steps involving the vector database introduce extra latency. This is a notable departure from traditional LQOs, which typically do not incur such overhead. Reducing this delay remains crucial for achieving real-time performance.

% \noindent\textbf{Complex Workload Evaluation:} 
% Future work should evaluate the model on more complex benchmarks to see {\oursystem}'s great potential in complicated queries, such as TPC-DS~\cite{tpcds} and RedBench~\cite{redbench}, to further validate its generalization capabilities and performance under diverse, real-world conditions.



\noindent\textbf{Close Integration of LLMs and Database Engine.} 
Embedding LLMs directly within the database engine potentially further minimizes latency by eliminating external calls~\cite{tian2019synergistic,kraska2018case}. \toreviewerone{OLAP queries typically require longer execution times than OLTP queries. The current additional overhead of {\oursystem} still poses challenges for its application in OLTP scenarios.} A closer integration may make this scenario possible.
Additionally, such integration may enable the LLM to support broader functionalities, including query optimization and query scheduling.


